Equidistribution of Dynamically Small Subvarieties over the Function Field of a Curve

For a projective variety X defined over a field K, there is a special class of self-morphisms of X called algebraic dynamical systems. In this paper we take K to be the function field of a smooth curve and prove that at each place of K, subvarieties of X of dynamically small height are equidistributed on the associated Berkovich analytic space. We carefully develop all of the arithmetic intersection theory needed to state and prove this theorem, and we present several applications on the non-Zariski density of preperiodic points and of points of small height in field extensions of bounded degree.

==> Fund_Ineq.tex <==
% Fundamental Inequality section of 
% ``Dynamically small points on function fields of curves''

\subsection{The Fundamental Inequality}
\label{Section: Fundamental Inequality}
	
	In this section we prove half of the function field analogue of Zhang's Theorem of the 
	Successive Minima, also known as the Fundamental Inequality. It was proved in this setting
	by Gubler, but we give an alternative proof using Siu's theorem.

	Let $X$ be variety of dimension $d$ defined over the function field $K$, and let $\met{L}$ be a 
	semipositive metrized line bundle on $X$ with ample underlying bundle $L$. Define the quantity
		\[
			e_1(X, \met{L}) = \sup_{\substack{V \subset X \\ \codim(V) = 1}} 
				\left\{ \inf_{x \in X\setminus V}  h_{\met{L}}(x) \right\}, 
		\]
	where the supremum is over all closed subsets $V$ of $X$ of pure codimension $1$, and the 
	infimum is over closed points of $X \setminus V$. 
		
\begin{thm}[Fundamental Inequality]
	\label{Thm: Succ Min}
	Let $X$ be variety of dimension $d$ defined over the function field $K$, and let $\met{L}$ be a 
	semipositive metrized line bundle on $X$ with ample underlying bundle $L$. Then
		\be
			e_1(X, \met{L}) \geq h_{\met{L}}(X).
		\ee
\end{thm}

	This inequality was originally discovered by Zhang when $K$ is a number field
	(see \cite{Zhang_Positive_Varieties_1995}), and it was proved by Gubler when $K$ is a function
	field in \cite{Gubler_Bogomolov_2007}. 
	
\begin{siu}[{\cite[Theorem~2.2.15]{Lazarsfeld_Positivity_2004}}] \label{Theorem: Siu}
	Let $\mathcal{Y}$ be a projective variety of dimension $n$ 
	over the field $k$ and suppose $\mathcal{N}_1$ and $\mathcal{N}_2$ are 
	nef line bundles on $\mathcal{Y}$. Then
		\[
			\dim_k H^0\left(\mathcal{Y}, \left(\mathcal{N}_1 \otimes 
				\mathcal{N}_2^{\vee}\right)^r \right) = \frac{\chern{\mathcal{N}_1}^n -n\ 
				\chern{\mathcal{N}_1}^{n-1}\chern{\mathcal{N}_2}}{n!} r^n + o(r^n).
		\] 
	In particular, if 
	$\chern{\mathcal{N}_1}^n -n\ \chern{\mathcal{N}_1}^{n-1}\chern{\mathcal{N}_2} > 0$, then 
	$\left(\mathcal{N}_1 \otimes \mathcal{N}_2^{\vee}\right)^{ r}$ has nonzero 
	global sections for $r \gg 0$.
\end{siu}

	We prove several preliminary lemmas that allow us to generate sections of models 
	approximating $\met{L}$.

\begin{lem} \label{Lem: Make it nef}
	Let $X$ be variety defined over the function field $K$ and $L$ a very ample line bundle on $X$. 
	Suppose $(\XX, \LL)$ is a $\BB$-model of $(X, L^e)$ such that $\LL$ is relatively semipositive 
	on $\XX$, and let $\pi: \XX \to \BB$ be the structure morphism. Then there 
	exists an ample line bundle $\mathfrak{b}$ on $\BB$ such that $\LL \otimes \pi^* \mathfrak{b}$ is 
	nef on $\XX$.
\end{lem}

\begin{proof}
	Choose a basepoint free basis of global sections $s_1, \ldots, s_n$ of $L$. By flatness, we may
	view each $s_i$ as a rational section of $\LL$. Write $[\Div(s_i)] = D_{i, 1} + D_{i,2}$, where 
	$D_{i,1}$ is a horizontal cycle on $\XX$ and $D_{i,2}$ is a vertical cycle. Then $D_{i,1}$ is effective
	for each $i$ since it is the closure of the cycle $[\Div(s_i|_X)]$. Choose closed points
	$v_1, \ldots, v_m \in \BB$ and positive integers $n_j$ such that $D_{i,2} + \sum_j n_j [\XX_{v_j}]$ is
	effective for all $i$. Set $\mathfrak{b} = \OO_{\BB}( \sum_j n_j [v_j])$.
	
	Let us first check that $\LL \otimes \pi^* \mathfrak{b}$ is still relatively semipositive.
	Let $\mathcal{C}$ be a curve on $\XX$ such that $\pi(\mathcal{C}) = \{v\}$ for 
	some closed point $v \in \BB$. As the base is a smooth curve, we may utilize a moving lemma
	in order to find a rational section $t \in \mathfrak{b}$ such that $v$ does not lie in the support
	of  $[\Div(t)]$. Therefore 
	$\chern{\pi^*\mathfrak{b}} \cdot \mathcal{C} = \pi^*[\Div(t)] \cdot \mathcal{C} = 0$. As $\LL$
	is relatively semipositive, we know by definition that $\chern{\LL} \cdot \mathcal{C} \geq 0$. 
	Combining these, we find $\chern{\LL \otimes \pi^* \mathfrak{b}} \cdot \mathcal{C} \geq 0$. 
		
	Now take $\mathcal{C}$ to be a horizontal curve on $\XX$. Then we can write 
	$\mathcal{C} = \overline{x}$ for some closed point $x$ on the generic fiber. Take one of the sections 
	$s_i$ such that $x \not\in \supp(s_i)$. Then $\mathcal{C}$ is not contained in the support of 
	$[\Div(s_i)]$. Moreover, since $D_{i,2} + \sum_j n_j [\XX_{v_j}]$ is effective, its intersection with 
	$\mathcal{C}$ must be nonnegative. Thus $\chern{\LL \otimes \pi^* \mathfrak{b}} \cdot \mathcal{C}
	\geq 0$.
\end{proof}

	As a passing remark, we should note that the proof of the lemma can be adapted using the 
	Kleiman-Nakai-Moishezon criterion to show that if
	$\LL$ is relatively ample on $\XX$, then $\LL \otimes \pi^* \mathfrak{b}$ is ample. 
	
\begin{lem} \label{Lem: Find some sections}
	Let $X$ be variety of dimension $d$ defined over the function field $K$ and $L$ an ample line bundle
	on $X$. Suppose $(\XX, \LL)$ is a $\BB$-model of $(X, L^e)$ such that $\LL$ is relatively 
	semipositive on $\XX$. Then
		\benn
			\dim_k H^0(\XX, \LL^r) \geq \frac{\chern{\LL}^{d+1}}{(d+1)!} r^{d+1} + O(r^d).
		\eenn
	In particular, $\LL^r$ has nonzero global sections for $r \gg 0$ if $\chern{\LL}^{d+1} > 0$.
\end{lem}	

\begin{proof}
	Let $\mathfrak{b}$ be a line bundle as in the previous lemma, and note that $\pi^*\mathfrak{b}$ 
	is nef on $\XX$. For ease of notation, let $\LL_1 = \LL \otimes \pi^* \mathfrak{b}$. Then Siu's
	Thoerem gives
		\be \label{Eqn: Siu expansion}
			\ba
				\dim_k H^0(X, \LL^r) &= 
					\dim_k H^0(X, \left(\LL_1 \otimes \pi^* \mathfrak{b}^{\vee}\right)^r) \\
				&\geq \frac{\chern{\LL_1}^{d+1} - (d+1) \chern{\LL_1}^d \chern{\pi^* \mathfrak{b}}}
					{(d+1)!} r^{d+1} + O(r^d).
			\ea
		\ee
	A moving lemma argument as in the proof of the previous lemma shows 
	$\chern{\pi^*\mathfrak{b}}^2 = 0$ as a functional on codimension-two cycles. Therefore
		\be \label{Eqn: Nef expansion}
			\ba
				\chern{\LL_1}^{d+1} = \chern{\LL \otimes \pi^*\mathfrak{b}}^{d+1}
				&= \chern{\LL}^{d+1} + (d+1)\chern{\LL}^d
					\chern{\pi^* \mathfrak{b}} \\
				&= \chern{\LL}^{d+1} + (d+1) \chern{\LL_1}^d\chern{\pi^*{\mathfrak{b}}}.
			\ea
		\ee
	Combining~\eqref{Eqn: Siu expansion} with~\eqref{Eqn: Nef expansion} gives the desired result.
\end{proof}
 
\begin{proof}[Proof of Theorem~\ref{Thm: Succ Min}]
	We firstreduce to proving that if $\met{L}$ is a semipositive metrized line
	bundle on $X$ with if $h_{\met{L}}(X) > 0$, then
	$e_1(X, \met{L}) \geq 0$. For suppose we know this, and suppose further that there exists 
	a semipositive metrized line bundle $\met{L}$ such that  $e_1(X, \met{L}) < h_{\met{L}}(X)$. 
	Fix a place $v$ of $K$ and choose a real number $a$ such that 
	$e_1(X, \met{L})+a[k(v):k] < 0 < h_{\met{L}}(X) + a[k(v):k]$. By 
	Theorem~\ref{Thm: General Heights}(ii), we
	find that $\met{L} \otimes \met{O_X(a)}$ is semipositive and $e_1(X, \met{L} \otimes \met{O_X(a)})
	< 0 < h_{\met{L} \otimes \met{O_X(a)}}(X)$. This inequality stands in contradiction to our hypothesis.
	
	Now let us prove that $h_{\met{L}}(X) > 0$ implies $e_1(X, \met{L}) \geq 0$. Replacing $\met{L}$
	by $\met{L}^m$ scales all heights by $m$, so we may reduce to the case that $L$ is very ample on
	$X$. Fix $\varepsilon > 0$ and a $\BB$-model $(\XX, \LL)$ of $(X, L^e)$ such that
		\begin{itemize}
			\item $\LL$ is relatively semipositive,
			\item $\sum_v [k(v):k] 
				\dist_v \left(\metric_{\LL, v}^{1/e}, \metric_{\met{L},v}\right) \leq \varepsilon$, and 
			\item $\chern{\LL}^{d+1} > 0$.
		\end{itemize}
	We may accomplish all of these things by definition of a semipositive metrized line bundle and 
	by continuity of arithmetic intersection numbers with respect to change of metric 
	(\xhelp{Point to the new approximation lemma}). By Lemma~\ref{Lem: Find some sections}, 
	there exists a positive integer $r$ and a nonzero global section $s$ of $\LL^r$. Choose
	$x \in X$ a closed point with $\overline{x}$ not contained in the support of $s$. Then
	$\chern{\LL}\cdot [\overline{x}] \geq 0$. By Theorem~\ref{Theorem: Intersection properties}(ii), 
	we have
		\benn
			\ba
				\achern{\met{L}|_x} &\geq \frac{\chern{\LL}\cdot [\overline{x}]}{e} - 
					\varepsilon \deg(x)	 \geq - \varepsilon \deg(x) \\
				&\Rightarrow h_{\met{L}}(x) \geq -\varepsilon \\
				&\Rightarrow \inf_{x \not\in \supp(s|_X)} h_{\met{L}}(x) \geq - \varepsilon \\
				&\Rightarrow e_1(X, \met{L}) \geq -\varepsilon.
			\ea
		\eenn
	Letting $\varepsilon \to 0$ proves $e_1(X, \met{L}) \geq 0$, and we are finished showing the
	first inequality of the theorem.
\end{proof}

\begin{comment}
	Now we state a conjectured generalization of the Fundamental Inequality. It turns out to be
	exactly the right ingredient to prove an equidistribution theorem; see Theorem~\xhelp{Point to 
	the general theorem in the equi proof section}.
	Let $X$ be a projective variety over the function field $K$ and $\met{L}$ a semipositive metrized
	line bundle on $X$ with ample underlying bundle $L$. For a collection $\F$ of 
	proper subvarieties of $X$, define
		\[
			e_1(X, \met{L}, \F) = \sup_{\substack{V \subset X \\ \codim(V) = 1}} 
				\left\{ \inf_{\substack{Y \in \F \\ Y \not\subset V}} h_{\met{L}}(Y) \right\}, 
		\]
	where the supremum is over all closed subsets $V$ of $X$ of pure codimension $1$, and the 
	infimum is over subvarieties $Y \in \F$ not contained in $V$. For example, if $\F$ is the collection
	of closed points of $X$, then $e_1(X, \met{L}, \F) = e_1(X, \met{L})$. 
	We expect this quantity to behave very much like $e_1(X, \met{L})$ in the Fundamental Inequality:
	
\begin{conjecture}
	Let $X$ be variety of dimension $d$ defined over the function field $K$, and let $\met{L}$ be a 
	semipositive metrized line bundle on $X$ with ample underlying bundle $L$. Then
		\benn
			e_1(X, \met{L}, \F) \geq h_{\met{L}}(X) 
		\eenn
\end{conjecture}

	\xhelp{Comment on the cases where we know the conjecture: $\F = points$ and $\met{L}$ arising
		from dynamical systems.}
\end{comment}
